An Emulator for Fine-Tuning Large Language Models using Small Language Models

Widely used language models (LMs) are typically built by scaling up a two-stage training pipeline: a pre-training stage that uses a very large, diverse dataset of text and a fine-tuning (sometimes, 'alignment') stage that uses targeted examples or other specifications of desired behaviors. While it has been hypothesized that knowledge and skills come from pre-training, and fine-tuning mostly filters this knowledge and skillset, this intuition has not been extensively tested. To aid in doing so, we introduce a novel technique for decoupling the knowledge and skills gained in these two stages, enabling a direct answer to the question, "What would happen if we combined the knowledge learned by a large model during pre-training with the knowledge learned by a small model during fine-tuning (or vice versa)?" Using an RL-based framework derived from recent developments in learning from human preferences, we introduce emulated fine-tuning (EFT), a principled and practical method for sampling from a distribution that approximates (or 'emulates') the result of pre-training and fine-tuning at different scales. Our experiments with EFT show that scaling up fine-tuning tends to improve helpfulness, while scaling up pre-training tends to improve factuality. Beyond decoupling scale, we show that EFT enables test-time adjustment of competing behavioral traits like helpfulness and harmlessness without additional training. Finally, a special case of emulated fine-tuning, which we call LM up-scaling, avoids resource-intensive fine-tuning of large pre-trained models by ensembling them with small fine-tuned models, essentially emulating the result of fine-tuning the large pre-trained model. Up-scaling consistently improves helpfulness and factuality of instruction-following models in the Llama, Llama-2, and Falcon families, without additional hyperparameters or training.

==> history/intro.tex <==
Unsupervised pre-training of large language models on massive, diverse datasets of text followed by human-supervised `alignment' with high-quality human-written demonstrations and preference annotations has proven to be a powerful recipe for building generally capable language systems [cite GPT-4, Claude, PaLM, Llama-2?].
%%CF.9.23: This sentence is a mouthful. Maybe break it into two sentences.
The strongest of these systems have demonstrated surprising skill at reasoning [chain of thought et al], general world knowledge [GPT-4], tool use [meta paper, GPT-4], and arithmetic [cite GPT-3, others]. While a widely-held hypothesis is that pre-training imbues a model with general knowledge and skills, while fine-tuning or alignment generally `filters' or `redirects' these learned behaviors toward the desired task or values,
%%CF.9.23: double "while" prepositional phrases is really awkward and confusing to read.
rigorous experimental validation of this hypothesis is limited [cite reward overoptimization].
%%CF.9.23: I feel like this is way too early to be mentioning the method and contributions, and generally makes this paragraph cover too many different things. I'd suggest keeping this paragraph to be about the motivation and problem. 
%%CF.9.23: You talk about the limited validation/understanding of the role of pre-training and fine-tuning above, but don't provide much else in terms of motivation. The method is a core part of the contribution, so this motivation needs to also outline the problem that the method solves, so that the method is well-motivated.
In this paper, we introduce a simple framework for \textit{scale-decoupled} language models, which leverages recent theoretical developments in reinforcement learning in language models to directly study the benefits of scaling pre-training and alignment independently. In addition, we demonstrate that when the computational cost of fine-tuning large open-source pre-trained models is prohibitive, scale-decoupled language models enable \textit{up-scaling} a small fine-tuned language model without any fine-tuning to achieve much of the benefits that \textit{would have} been achieved by fine-tuning the larger pre-trained model.
%%CF.9.23: It would be nice to be upfront about the fact that this only applies to RLHF-based fine-tuning/alignment/steering (and not supervised fine-tuning)

% - The specific recipe of pre-training + fine-tuning has been really successful, and predicting when model capabilities will show up has proven difficult [cite emergence stuff?]
% - While a widely-held hypothesis is that pre-training imbues a model with general knowledge, while fine-tuning or alignment generally `filters' or `redirects' these learned behaviors, rigorous experimental validation of this hypothesis is limited [cite reward overoptimization]
% - In this paper, we will introduce a simple framework for `scale-decoupled' language models, which leverages recent theoretical developments in reinforcement learning in language models to directly study the benefits of scaling pre-training and alignment independently
% - In addition, we demonstrate that when the computational requirements of fine-tuning large open-source pre-trained models are prohibitive, scale-decoupled language models enable `up-scaling' a small fine-tuned language model without any fine-tuning to achieve much of the benefits that \textit{would have} been achieved by fine-tuning the larger pre-trained model.

Our analysis is built on the framework of scale-decoupled language models,
%%CF.9.23: This sentence seems to imply that this framework existed before this paper.
which is a principled approach to combining the knowledge learned by a pre-trained model of one size with the knowledge learned \textit{during fine-tuning only} by a different model of another size. 
%%CF.9.23: They don't necessarily need to be of different sizes
The framework uses a reinforcement learning perspective on fine-tuning based on the language model-reward function duality presented by \citet{rafailov2023direct}, but it is applicable to any fine-tuned language model whether or not reinforcement learning was used.
%%CF.9.23: I generally feel like this presentation is not all that intuitive. At this point, I think the reader won't really understand the duality that you referenced above nor what scale-decoupled models actually are. Can you try to build up these concepts gradually?
Crucially, scale-decoupled models can be explicitly constructed with off-the-shelf language models and sampled from efficiently; while they share some similarities to methods such as contrastive decoding [cite], our principled formulation eliminates the need for any new hyperparameters to achieve quality samples. Thus, scale-decoupled models enable the study of independent scaling of pre-training and fine-tuning. 
%%CF.9.23: I still don't think that the reader will know what scale-decoupled models are here.
Through our analysis of scale-decoupled language models, we find evidence across three model families and two open-ended instruction following datasets supporting the intuition that pre-training at scale enables greater accumulating of raw knowledge (improved factual correctness), while fine-tuning at larger scale produces greater helpfulness (improved user satisfaction).
%%CF.9.23: Seems a little early to be mentioning experiments. it may be helpful to try to start with an outline for the intro before the next draft. Because there are multiple contributions, the organization might be a little trickier than a typical methods-focused intro, and I'm not sure if the current organization is optimal.
% Scale-decoupled models are based on an interpretation of \textit{any} LM as the result of fine-tuning a pre-trained model with reinforcement learning (RL), using a specifically-constructed reward function and a KL constraint to the pre-trained model.\footnote{While this interpretation is based on an RL framework, it applies to any language model, even if it is fine-tuned with supervised learning, not RL.} This interpretation is possible due to the language model-reward function duality described by \citet{rafailov2023direct}. In the scale-decoupled formulation, the reference model represents the information absorbed from pre-training, and the reward function represents the information absorbed from fine-tuning. Be

% This formulation allows us to make explicit that a given fine-tuned language model is the result of two separate learning processes: a pre-training process that produces the base model, and a fine-tuning (or alignment) process that produces the final LM., we have a principled basis to construct a conditional distribution that simulates the result of pre-training at one scale and fine-tuning (or `aligning') at another scale.
% - Sampling from the resulting scale-decoupled language model enables us to study the results of scaling pre-training and fine-tuning independently
% - We find evidence across three model families and two open-ended instruction following datasets supporting the intuition that pre-training at scale enables greater accumulating of raw knowledge (improved factual correctness), while fine-tuning at larger scale produces greater helpfulness (improved user satisfaction)

Beyond this scientific finding, we also find that scale-decoupled language models enable boosting the performance of small fine-tuned models by a process we call \textit{up-scaling}, essentially ensembling them with newer, larger pre-trained models, without any fine-tuning or modifications to either model. Our experiments show that up-scaling a small fine-tuned policy (e.g., 7B) with a newer, larger pre-trained base model (e.g. 180B) provides the majority of the improvements in factuality that \textit{would} be achieved by fine-tuning the larger pre-trained model (e.g. 180B). Up-scaling also consistently improves the average response helpfulness, as rated by GPT-4. In scenarios where fine-tuning a small language model is viable (e.g. Falcon-7B) but fine-tuning a larger language model is not (e.g., Falcon-180B), due to resource constraints, up-scaling enables capturing much of the benefits of fine-tuning the larger model, without performing any model fine-tuning at all.
%- Our experiments also show that up-scaled LMs work without any hyperparameter tuning at all.%, an improvement over existing methods like Contrastive Decoding [cite].

In summary, our primary contributions are: 
\begin{enumerate}
    \item The \textit{scale-decoupled} language model framework, which enables studying the benefits of scaling pre-training and fine-tuning separately;
    \item Clear experimental support for the hypothesis that scaling pre-training contributes to increased model knowledge, while scaling fine-tuning contributes to more helpful instruction-following; and
    \item The technique of \textit{model up-scaling}, which enables a small fine-tuned model and large base model to approximate the compute-intensive result of fine-tuning a large base model.
\end{enumerate}
